Beyond Token Savings: A Systematic Study of Context Compression in LLM Agents

As LLM agents tackle longer tasks, they increasingly compress growing histories of reasoning, actions, and tool outputs. Compression can reduce token use, but it also changes the information available for later decisions. Existing agentic harnesses bundle decisions about what to compress, when to compress, and how much to remove into fixed policies. A systematic characterization is needed to disentangle these decisions and reveal how each affects task success and execution cost. We systematically vary these decisions across three open-weight models on SWE-bench Verified and Terminal-Bench 1.0. Across nearly 35,000 agent runs, we measure task success, token use, end-to-end latency, and estimated cost. We find that fewer tokens need not mean faster or cheaper execution: on Terminal-Bench with Qwen, policies using roughly one-third as many tokens can take 20-80% longer than the uncompressed agent. Policies with similar overall success can solve different tasks, while the same policy can perform quite differently across models. Our results motivate evaluating compression by its effects on agent execution and tailoring policies to the task, model, and workload.

==> sections/05-RelatedWorks.tex <==
\section{Related work}

\noindent\textbf{Prior agentic serving characterization.}
Long agent trajectories can become difficult to serve effectively even before reaching the model's context limit. 
Prior work shows that models make weaker use of distant information and often incur increasing token overhead as context grows~\citep{packer2023memgpt, hu2025hiagent, liu2024lost, tian2025distance, du2025context}. 
Recent characterization studies examine related effects at different levels: multi-turn performance degradation in LLMs~\citep{laban2026llms}, end-to-end execution\citep{kim2026dynamicreasoning, raj2026cpucentric, chang2026agentsysbench}, resource usage \citep{yang2026agora, zheng2026agentcgroup}, and serving behavior of agents\citep{kondrashov2026aries, kim2026gaiatrace, yuan2026workloadchar, yuan2026kairos}, and production-scale workload, context growth, and cache behavior in GitHub Copilot~\citep{liu2026agentic}. 
Together, these works establish that growing agent context affects both model behavior and serving efficiency. 
However, they characterize workloads under a given context-management mechanism rather than systematically studying the compression policy itself. 
Our work instead varies \emph{what} is compressed, \emph{when} compression is triggered, and \emph{how aggressively} history is compressed, and measures how these choices change task success, execution length, cost, and latency.

\noindent\textbf{Context management inside the agent loop.}
Modern agents increasingly manage growing histories by truncating observations, summarizing earlier interactions, or combining both~\citep{codex_compaction, claude_context_editing, gemini_cli_compression, copilot_compaction, openhands_condenser, cline_compaction}. 
These mechanisms are already consequential in production: across 13 million Copilot sessions, sessions that invoke compaction account for 44\% of served tokens, and the median compaction removes 73\% of the context~\citep{liu2026agentic}.

Recent work proposes compression techniques that substantially reduce retained context while often preserving task success~\citep{kang2025acon, chen2026coact, lindenbauer2025complexity, xiao2026reducing}. 
However, compression can also alter the execution itself: agents may take additional steps, revisit discarded information, or incur extra model calls to construct summaries~\citep{min2026toward, lindenbauer2025complexity}. 
Consequently, evaluating compression only by the number of tokens removed can miss important downstream effects. 
We build on this observation by treating compression as a policy with separable design choices (primitive, trigger, and depth) and studying how each shapes the resulting agent trajectory across models and task environments.

\noindent\textbf{Serving efficiency and end-to-end cost.}
Prompt size is also an incomplete proxy for serving cost. Modern serving systems reuse KV state and shared prompt prefixes to reduce the cost of repeated context~\citep{kwon2023efficient}, while commercial APIs similarly discount cached input tokens~\citep{}. 
Compression can disrupt this reuse: rewriting earlier history may invalidate a cached prefix, while summarization itself introduces additional inference. 
Production Copilot traces observe reduced cache reuse around compaction~\citep{liu2026agentic}, and TokenPilot proposes prefix-stable compaction specifically to preserve reuse~\citep{xu2026tokenpilot}. 
As a result, reducing prompt tokens does not necessarily reduce either billed cost or end-to-end latency.

Our study connects these effects in a controlled evaluation of the compression policy itself. 
Rather than treating compression efficiency as the size of the compressed prompt, we evaluate the full execution it induces, including task outcome, token usage, number of agent steps, serving cost, and latency.
